Improving High Contention OLTP Performance via Transaction Scheduling

Research in transaction processing has made significant progress in improving the performance of multi-core in-memory transactional systems. However, the focus has mainly been on low-contention workloads. Modern transactional systems perform poorly on workloads with transactions accessing a few highly contended data items. We observe that most transactional workloads, including those with high contention, can be divided into clusters of data conflict-free transactions and a small set of residuals. In this paper, we introduce a new concurrency control protocol called Strife that leverages the above observation. Strife executes transactions in batches, where each batch is partitioned into clusters of conflict-free transactions and a small set of residual transactions. The conflict-free clusters are executed in parallel without any concurrency control, followed by executing the residual cluster either serially or with concurrency control. We present a low-overhead algorithm that partitions a batch of transactions into clusters that do not have cross-cluster conflicts and a small residual cluster. We evaluate Strife against the optimistic concurrency control protocol and several variants of two-phase locking, where the latter is known to perform better than other concurrency protocols under high contention, and show that Strife can improve transactional throughput by up to 2x. We also perform an in-depth micro-benchmark analysis to empirically characterize the performance and quality of our clustering algorithm

==> sections/problem.tex <==
\section{Problem Statement}
\seclabel{problem}
We defined the notion of an oracle scheduler in \secref{architecture} as a clustering algorithm that partitions a batch into conflict-free clusters and a residual cluster.

Such an oracle scheduler is not unique. For example, consider the partitionable variant\footnote{In this example, we consider only \texttt{New-Order} and \texttt{Payment} transactions without any remote payments or orders} of the TPCC workload. An algorithm (say $\mathcal{S}_1$) that clusters all transactions in the batch into a single conflict-free cluster is a trivial but correct scheduler. Similarly, an algorithm (say $\mathcal{S}_2$) that clusters all transactions belonging to the same warehouse together and those from different warehoses into different clusters. This scheduler produces $w$ (number of warehouses) clusters. Both these algorithms are correct oracle schedulers. However, $\mathcal{S}_2$ is preferred over $\mathcal{S}_1$ as it leads to a higher degree of parallelism during the \conflictfree phase. In this section, we qualify the oracle scheduler with a notion of optimality. 

The throughput of transaction processing in \system is inversely proportional to the average time taken to execute a single batch. The objective of a ``good" oracle scheduler is to minimize the total time taken to execute a batch of transactions $\mathcal{B}$. 

We formalize this optimization as a graph partitioning problem. Let $O$ be the set of objects in the database. Each transaction $T$ is represented as a pair $(D_T, A_T)$, where $D_T \subseteq O$ is the set of objects accessed by $T$ and $A_T: D_T \rightarrow \{\mathtt{r}, \mathtt{w}\}$ specifies the type of access for the corresponding data item, where \texttt{r} and \texttt{r} represent read and write accesses respectively. 

\paragraph{Conflict Graph} Given a batch of transactions $\mathcal{B}$, we define its corresponding conflict graph $\mathcal{C} = (\mathcal{B}, \mathcal{E})$ as a graph among transactions in the batch with an edge between two transactions $T$ and $T'$ when they have conflicting accesses to a data item. Specifically, edge $e = (T, T') \in \mathcal{E}$ when $\exists \ d \in D_T \text{ and } d \in D_{T'}$ such that either of the following is true:
\begin{myitemize}
\item $A_T(d) = \mathtt{r}$ and $A_{T'}(d) = \mathtt{w}$ 
\item $A_T(d) = \mathtt{w}$ and $A_{T'}(d) = \mathtt{r}$ 
\item $A_T(d) = \mathtt{w}$ and $A_{T'}(d) = \mathtt{w}$ 
\end{myitemize}

\guna{add an example here}

The oracle scheduler must partition the graph into $n$ conflict-free sets of vertices $C_1, C_2, ... C_n$ and a residual set of vertices $R$ such that the time taken to execute the batch is minimal. The execution time is the sum of time spent in the \analysis phase, \conflictfree phase and the \residual phase. It can be modeled as follows:
\begin{align*}
    t(\mathcal{B}) &= t(\analysis) + t(\conflictfree) + t(\residual) \\
    &= t(\analysis) + \eta_1 * \max_i(|C_i|) + \frac{\eta_2}{n} * |R|
\end{align*}
where $\eta_1$ is a constant that denotes average time taken to execute a transaction without concurrency control; and $\eta_2$ denotes the average time taken to execute a transaction with concurrency control. 

The key observation here is that execution time depends on two factors that result from the analysis: (1) the maximum size of the conflict-free clusters $\max_i(|C_i|)$ and (2) the size of the residual cluster $|R|$. Minimizing $t(\mathcal{B})$ can be posed as a multi-objective optimization problem that minimizes both $\max_i(|C_i|)$ and $|R|$. However, solving a multi-objective optimization problem is expensive. Since, time taken to solve this problem, $t(\analysis)$, adds to the total time to execute a batch, we simplify the problem by bounding one of the objectives. 

\paragraph{Bounded Outliers} We limit the number of transactions that are clustered into the residual cluster $R$ by bounding its size to a fraction of $|\mathcal{B}|$ using the parameter $\alpha$, where $0 \geq \alpha < 1 $. Parameter $\alpha$ controls the proportion of transactions that will be executed in the \conflictfree and \residual phases and the degree of parallelism in the \conflictfree phase. A higher value of $\alpha$ allows more spurious transactions to be clustered into residual cluster and this leads to a higher degree of parallelism in the \conflictfree phase; while a lower $\alpha$ value forces more of the spurious transactions to be included in the conflict-free clusters reducing the degree of parallelism during \conflictfree phase.\alvin{also talk about how to come up with $\alpha$.} 

Based on the above simplification, we pose the oracle scheduler optimization problem as follows: 
\begin{framed}
\begin{problemstatement*}
 Partition conflict-graph $\mathcal{C} = (\mathcal{B}, \mathcal{E})$ into $C_1, C_2, ... C_n$ and $R$ such that
\begin{equation*}
    \min_{R, C_1, .., C_k} \max_i(|C_i|)
\end{equation*}
where 
\begin{myenumerate}
\item $R, C_1, ..., C_k$ is a partition of $\mathcal{B}$
\item $\forall (T, T') \in \mathcal{E}$, we have $T \in C_i \implies T' \in C_i$
\item $|R| \leq \alpha * |\mathcal{B}|$
\end{myenumerate}
\end{problemstatement*}
\end{framed}

Condition $\S1$ ensures that all transactions in $\mathcal{B}$ are executed exactly once. $\S2$ is critical for serializability of transaction execution (refer \theref{serializability}) as the conflict-free clusters $C_1, ... C_n$ may be executed concurrently without concurrency control. $\S3$ bounds the size of residual clusters relative to the size of the batch. 

Further, the above model assumes unit cost for each transaction. This can be extended in a straight-forward way by assigning weights to transactions based on its computation cost or read-write set cardinality. 



